dots.tts.edit: Precisely Controlled Speech Editing with a Continuous Autoregressive Model

Speech editing for content creation requires precise control over both what an edit should do and where it should apply. Free-form natural language provides a flexible interface for expressing edit requests, but its ambiguity may leave the intended operation, parameters, or target region underspecified. We study a semi-formal transcript-grounded edit instruction that specifies operation categories and parameters and binds them to transcript spans or boundaries. This semantic timeline avoids explicit timestamp alignment and provides an externally inspectable contract for compositional edits. We instantiate the interface in dots$.$tts$.$edit, a speech editing model built on a continuous autoregressive speech generation architecture. Four representative speech-creation controls cover lexical content, affective expression, pitch and speaking-rate delivery, and temporal phrasing through text, emotion, prosody, and pause editing. Task-specific data pipelines construct operation- and scope-controlled pairs while retaining source-derived context outside each target region. We further introduce doteBench, a bilingual benchmark that measures precise instruction following, local preservation, and audio quality across the four controls and their composition. Experiments show leading overall instruction following and local preservation across its five editing categories, while audio quality remains comparable to existing open-source systems. Across three Seed-TTS-Eval shards, the model shows negligible differences from the base model in zero-shot TTS recognition error rate and speaker similarity.

==> figures/front-radar.tex <==
\par\medskip
\begin{minipage}{\textwidth}
  \centering
  \captionsetup{hypcap=false}
  \includegraphics[width=0.80\textwidth]{radar_editing_one_take_wide.pdf}
  \captionof{figure}{\textbf{Speech editing performance across five categories.}
  Each request is completed in a single generation pass. Farther from the
  center indicates better results on each metric. Axes measure how well
  systems follow the requested changes, preserve unedited speech, and
  maintain audio quality.}
  \label{fig:front-radar}
\end{minipage}
\par


==> title-page.tex <==
\font\reportwordmark="[fonts/RobotoSlab-Bold.otf]" at 18pt
\renewcommand{\dotsttsedittitle}{%
  \texorpdfstring{{\reportwordmark dots.tts.edit}}{dots.tts.edit}}
\makeatletter
\abstracttitle{\makebox[\textwidth][c]{Abstract}}
\renewcommand{\theaffn}{\arabic{affn}}
\renewcommand{\fnref}[1]{\def\@fnmark{\textdagger}}
\newcommand{\reportFirstPageNotes}{%
  \begingroup
    \long\def\footnotetext##1{\gdef\reportInternNote{##1}}%
    \@fnotes
    \long\def\footnotetext##1{\gdef\reportCorrespondingNote{##1}}%
    \@cornotes
  \endgroup
  \begingroup
    \let\thefootnote\relax
    \footnotetext{%
      \textsuperscript{\textdagger}\reportInternNote\quad
      \textsuperscript{*}\reportCorrespondingNote\par
      \textit{Email addresses: }\@elseads}%
  \endgroup}
\renewcommand{\maketitle}{%
  \raggedbottom
  \onecolumn
  \resetTitleCounters
  \begingroup
  \def\baselinestretch{1}%
  \setlength{\parskip}{0pt}%
  \begin{center}
    {\fontsize{18}{22}\selectfont\bfseries\@title\par}
    \vspace{10pt}
    {\fontsize{12}{14}\selectfont\bfseries
      \let\reportauthorSuperscript\textsuperscript
      \renewcommand{\textsuperscript}[1]{%
        \reportauthorSuperscript{\mdseries##1}}%
      \elsauthors\par}
    \vspace{8pt}
    {\fontsize{11}{13}\selectfont\normalfont\elsaddress\par}
    \paperresources
  \end{center}
  \vspace{14pt}
  \hrule\vspace{8pt}
  \ifvoid\absbox\else\unvbox\absbox\par\vspace{6pt}\fi
  \ifvoid\keybox\else\unvbox\keybox\par\vspace{6pt}\fi
  \hrule
  \input{figures/front-radar}
  \par
  \endgroup
  \def\@elseads{\texttt{wanghankun@xiaohongshu.com; \{wanghankun,kai.yu\}@sjtu.edu.cn}}%
  \reportFirstPageNotes
  \thispagestyle{plain}
  \gdef\thefootnote{\arabic{footnote}}%
  \clearpage
  \twocolumn[{%
    \begin{minipage}{\textwidth}
    \input{figures/instruction_example}
    \end{minipage}\par\vspace{14pt}}]
  \raggedbottom}
\makeatother

